Optimized Cost Per Click in Online Advertising: A Theoretical Analysis

In recent years, Optimized Cost Per Click (OCPC) and Optimized Cost Per Mille (OCPM) have emerged as the most widely adopted pricing models in the online advertising industry. However, the existing literature has yet to identify the specific conditions under which these models outperform traditional pricing models like Cost Per Click (CPC) and Cost Per Action (CPA). To fill the gap, this paper builds an economic model that compares OCPC with CPC and CPA theoretically, which incorporates out-site scenarios and outside options as two key factors. Our analysis reveals that OCPC can effectively replace CPA by tackling the problem of advertisers strategically manipulating conversion reporting in out-site scenarios where conversions occur outside the advertising platform. Furthermore, OCPC exhibits the potential to surpass CPC in platform payoffs by providing higher advertiser payoffs and consequently attracting more advertisers. However, if advertisers have less competitive outside options and consistently stay in the focal platform, the platform may achieve higher payoffs using CPC. Our findings deliver valuable insights for online advertising platforms in selecting optimal pricing models, and provide recommendations for further enhancing their payoffs. To the best of our knowledge, this is the first study to analyze OCPC from an economic perspective. Moreover, our analysis can be applied to the OCPM model as well.

==> sections/00.abstract.tex <==
\begin{abstract}
% TBD
% The online advertising industry is evolving rapidly, leading to the emergence of new pricing models such as Optimized Cost Per Click (OCPC) and Optimized Cost Per Mille (OCPM). 
Optimized Cost Per Click (OCPC) and Optimized Cost Per Mille (OCPM) have emerged as the most widely adopted online advertising pricing models in practice, with expectations of higher advertising platform payoffs.
However, the existing literature lacks a comprehensive understanding of the conditions under which these pricing models can outperform others. 
To this end, in this paper, we propose a game-theoretic approach to compare OCPC with traditional pricing models, namely Cost Per Click (CPC) and Cost Per Action (CPA). 
Our analysis indicates that OCPC effectively replaces CPA by tackling the problem of advertisers strategically manipulating conversion reporting, especially in cases where conversions occur outside the advertising platform. 
Furthermore, OCPC exhibits the potential to surpass CPC in platform payoffs by providing higher advertiser payoffs and consequently attracting more advertisers. 
% Additionally, OCPC has the potential to outperform CPC in terms of performance by attracting a greater number of advertisers and providing higher advertiser payoffs. 
However, if advertisers have limited competitive options outside the platform and consistently choose the focal platform, the platform may achieve higher payoffs using CPC. 
This research provides valuable insights for online advertising platforms in selecting optimal pricing models and offers recommendations to further enhance their payoffs. 
Moreover, the analysis in this study can be applicable to the OCPM model as well.

% Zixuan is all you need

% \yzx{
% % Pricing models in online advertising aim to synchronize the interests of advertisers and publishers, allowing for a fair exchange of value in terms of business goals and advertising revenues. 
% Pricing models in online advertising aim to facilitate a fair exchange of value between the business objectives of advertisers and advertising revenues of publishers. 
% Despite the rapid evolution of pricing models, little attention has been devoted to a comprehensive understanding of the bid auction conditions under which these models are superior to others.
% To this end, in this paper, we propose a game-theoretic approach to investigate the impact of bid auction conditions on the efficacy of Optimized Cost Per Click (OCPC) compared to two traditional pricing models, namely Cost Per Click (CPC) and Cost Per Action (CPA). 
% Our analysis shows that OCPC effectively replaces CPA by tackling the problem of advertisers strategically manipulating conversion reporting, especially in cases where conversions occur outside the advertising platform. 
% Furthermore, OCPC exhibits the potential to surpass CPC in performance by attracting more advertisers and providing higher advertiser payoffs. 
% % One caveat is that if advertisers face limited competitive options outside the platform and consistently choose the focal platform, the platform may achieve higher payoffs using CPC. 
% More importantly, our approach has provided theoretical guarantee on the optimal selection of pricing models under specified conditions, which ultimately enhances the payoffs of online advertising platforms. 
% We also demonstrate that our approach can be easily adapted to investigate other SOTA pricing models (e.g., OCPM) xxx.
% }

% Prof.Xiong is all you need

% As the online advertising industry rapidly evolves, new pricing models such as Optimized Cost Per Click (OCPC) and Optimized Cost Per Mille (OCPM) have emerged as crucial components. However, the existing literature lacks an understanding of why and when these models can outperform others. In this study, we employ a game-theoretic approach to compare OCPC with traditional pricing models, Cost Per Click (CPC) and Cost Per Action (CPA). Our findings reveal that OCPC effectively substitutes CPA by addressing the issue of advertisers strategically manipulating conversion reporting, particularly in scenarios where conversions occur outside the advertising platform. Furthermore, OCPC can surpass CPC in performance by attracting more advertisers and offering a higher advertiser payoff. Nevertheless, a platform may still achieve a higher payoff using CPC when advertisers have less competitive outside options and consistently choose the focal platform. This research offers valuable insights for online advertising platforms in selecting optimal pricing models and provides recommendations for enhancing their payoffs. Additionally, our analysis is also applicable to the OCPM model.

% GPT4 is all you need

% Online advertising pricing models continue to iterate with the rapid evolution of the online advertising industry. The most recent ones, Optimized Cost Per Click (OCPC) and Optimized Cost Per Mille (OCPM) have quickly become the most important pricing models since their invention. However, it is still unclear in the literature why and when they can dominate other pricing models. In this paper, we build a game theoretic model to compare OCPC with Cost Per Click (CPC) and Cost Per Action (CPA). We find that OCPC substitutes for CPA because OCPC can solve the problem of advertisers strategically manipulating conversion reporting, which applies to the broader out-site scenario where conversions occur outside of advertising platforms. In addition, OCPC can outperform CPC by attracting more advertisers with a higher advertiser payoff. However, a platform can have a higher payoff with CPC if advertisers have no competitive outside options and always choose the focal platform. Our paper provides guidance for online advertising platforms to choose appropriate pricing models. We also provide suggestions for platforms to further increase their payoffs. Our analysis also applies to OCPM.
\end{abstract}
